Compact Trilinear Interaction for Visual Question Answering

In Visual Question Answering (VQA), answers have a great correlation with question meaning and visual contents. Thus, to selectively utilize image, question and answer information, we propose a novel trilinear interaction model which simultaneously learns high level associations between these three inputs. In addition, to overcome the interaction complexity, we introduce a multimodal tensor-based PARALIND decomposition which efficiently parameterizes trilinear interaction between the three inputs. Moreover, knowledge distillation is first time applied in Free-form Opened-ended VQA. It is not only for reducing the computational cost and required memory but also for transferring knowledge from trilinear interaction model to bilinear interaction model. The extensive experiments on benchmarking datasets TDIUC, VQA-2.0, and Visual7W show that the proposed compact trilinear interaction model achieves state-of-the-art results when using a single model on all three datasets.

==> compare-sota.tex <==
\subsection{Comparison with the state of the art}

\begin{table*}[!t]
\centering
%\footnotesize
\small
\begin{tabular}{c|c|cccccccc|cccc}
\hline
\multirow{2}{*}{\textbf{Dataset}}              & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Metrics\end{tabular}}} & \multicolumn{12}{c}{\textbf{Reference models}}                                                                                                             \\ \cline{3-14} 
                                               &                                                                                       & \textbf{\begin{tabular}[c]{@{}c@{}}BAN2\\ \cite{Kim2018BilinearAN}\end{tabular}}  & \textbf{\begin{tabular}[c]{@{}c@{}}BAN8\\ \cite{Kim2018BilinearAN}\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}SAN\\ \cite{Yang2016StackedAN}\end{tabular}} &\textbf{\begin{tabular}[c]{@{}c@{}}QTA\\ \cite{MTL_QTA}\end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}MCB\\ \cite{Fukui2016MultimodalCB}\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}RAU\\ \cite{noh2016training}\end{tabular}}& \textbf{BAN2-TI} & \textbf{BAN8-TI} & \textbf{\begin{tabular}[c]{@{}c@{}}MLP\\ \cite{jabri2016revisiting}\end{tabular}} &\textbf{\begin{tabular}[c]{@{}c@{}}fPMC\\ \cite{hu2018learningfPMC}\end{tabular}}  &  \textbf{\begin{tabular}[c]{@{}c@{}}STL\\ \cite{wang2018structuredSTL}\end{tabular}}& \textbf{CTI} \\ \hline
\multirow{4}{*}{\textbf{TDIUC}} 
% & \textbf{Acc}                                                                            & 86.3           & 82.3           & 85.0         & 79.2         & 84.3         & 87.3            & \_           & \_            & \_           & \_           \\ 
                                               & \textbf{Ari}                                                                             &67.4     & 67.9           & 65.0          & 69.1         & 65.8         & 67.8         & 72.5      & \textbf{73.2}      & \_           & \_            & \_           & \_           \\  
                                               & \textbf{Har}                                                                            &54.9     & 56.8           & 53.7           & 60.1         & 58.0         & 59.0         & 65.5     & \textbf{66.9}       & \_           & \_            & \_           & \_           \\ 
                                               & \textbf{Ari-N}                                                                          &37.4     & 35.9           & 35.4           & \_           & 39.8         & 41.0         & \textbf{45.8}      & 44.9      & \_           & \_            & \_           & \_           \\ 
                                               
                                               & \textbf{Har-N}                                                                          &15.7     & 13.9           & 14.7           & \_           & 24.8         & 24.0         & \textbf{28.6}     & 25.2       & \_           & \_            & \_           & \_           \\ \hline
% \textbf{VQA-2.0 test-dev set}                  & \textbf{Acc}                                                                            & 70.04          & xx.x           & \_           & 62.3         & \_           & xx.x            & \_           & 63.9          & \_           & \_           \\ \hline
\textbf{V7W}                     & \textbf{Acc}                                                                            & \_             & \_             & \_           & \_           & \_     & 62.2         & \_       & \_       & 67.1         & 66.0          & 68.2         & \textbf{72.3}         \\ \hline
% \textbf{VQA-1.0 MC test-dev set}               & \textbf{Acc}                                                                            & \_             & \_             & \_           & \_           & \_           & \_              & 65.2         & \_            & 69.7         & xx.x         \\ \hline
\end{tabular}
\caption{Performance comparison in TDIUC validation and and Visual7W validation set. \textbf{BAN2-TI} and \textbf{BAN8-TI} are denoted as student models trained under our compact trilinear interaction teacher model used for Free-form Opended-ended VQA task. \textbf{BAN8} is also used for comparison due to the state-of-the-art result is reported in this version of BAN \cite{Kim2018BilinearAN}. \textbf{CTI} is denoted as proposed compact trilinear interaction model, which is used for Multiple-Choice VQA task. The omitted ones are due to their missing in the corresponding work. Noting that to have an explicitly comparison, we train BAN and SAN models with there best setting in all testing dataset.}
\label{tab:exp_sota}
\end{table*}

To compare the performance of the proposed approach to the state of the art, we associate CTI with recently introduced techniques for VQA, which are then described below.

\textbf{Attention mechanism.} We use the tri-attention distribution map proposed in Section \ref{Sec:proposal} and apply residual glimpse introduced in \cite{Kim2018BilinearAN} which value is set as $8$. For Free-form Opened-ended VQA task, BAN with glimpse $8$ is applied as student model of the proposed trilinear interaction teacher model. 

\textbf{Input features.} There are no changes for word embedding mechanism introduced in Section \ref{Sub:Exp_dataset}. However, visual features will be extracted by Bottom Up \cite{bottom-up2017} for both Free-form Opened-ended and Multiple-choice VQA task due to its effectiveness has been proved in \cite{bottom-up2017, Kim2018BilinearAN, MTL_QTA}.

\textbf{Results.} State-of-the-art comparison results are gathered in Table.\ref{tab:exp_sota} for both Free-form Opened-ended and Multiple-choice VQA task. Among all introduced settings, our proposed CTI outperform the corresponding classification model by a noticeable margin in all mentioned evaluation metrics. Noting that there are differences on the experimental setups in many of the comparison to state-of-the-art methods. With our best proposed setting, our model outperforms current state-of-the-art QTA \cite{MTL_QTA} in TDIUC validation set by $4.1\%$ on Arithmetic MPT metric and by $6.8\%$ on Harmonic MPT metric, i.e. both metrics are important for evaluation on TDIUC dataset. In Visual7W test set, proposed model also beats current state-of-the-art STL \cite{wang2018structuredSTL} by a large margin - upto $4.1\%$ (from $68.2\%$ to $72.3\%$). Visualization of CTI are showed in Fig.\ref{fig:vis_CTI}. Noting that the visualize results are get from test set of Visual7W.
\begin{figure}
    \centering
    \includegraphics[width = \columnwidth, keepaspectratio=True]{ICCV2019_AIOZ/images/Visualization.pdf}
    \caption{Visualization of proposed CTI which learn joint representation over channels of visual, question and answer based on trilinear attention distribution map.}
    \label{fig:vis_CTI}
\end{figure}

